TaskCLIP: Extend Large Vision-Language Model for Task Oriented Object Detection

Task-oriented object detection aims to find objects suitable for accomplishing specific tasks. As a challenging task, it requires simultaneous visual data processing and reasoning under ambiguous semantics. Recent solutions are mainly all-in-one models. However, the object detection backbones are pre-trained without text supervision. Thus, to incorporate task requirements, their intricate models undergo extensive learning on a highly imbalanced and scarce dataset, resulting in capped performance, laborious training, and poor generalizability. In contrast, we propose TaskCLIP, a more natural two-stage design composed of general object detection and task-guided object selection. Particularly for the latter, we resort to the recently successful large Vision-Language Models (VLMs) as our backbone, which provides rich semantic knowledge and a uniform embedding space for images and texts. Nevertheless, the naive application of VLMs leads to sub-optimal quality, due to the misalignment between embeddings of object images and their visual attributes, which are mainly adjective phrases. To this end, we design a transformer-based aligner after the pre-trained VLMs to re-calibrate both embeddings. Finally, we employ a trainable score function to post-process the VLM matching results for object selection. Experimental results demonstrate that our TaskCLIP outperforms the state-of-the-art DETR-based model TOIST by 3.5% and only requires a single NVIDIA RTX 4090 for both training and inference.

==> backup_intro.tex <==
Traditional object detection algorithms are primarily designed to identify object instances belonging to predefined categories within an image. 
These algorithms focus on finding all object items given a image and performing classification over each item. However, in real-world applications, such as intelligent service robotics, the challenge is to find suitable objects based on different requirements instead of detecting all objects. 
This requires models to first analyze text requirements, such as ``\textit{sit comfortably}'', and then find the optimal item, such as ``\textit{chair}''. Given this task requirement, the work~\cite{sawatzky2019object} introduces the concept of ``\textit{task-oriented object detection}'' and propose a new dataset called COCO-Tasks which is based on traditional MS COCO 2014~\cite{lin2014microsoft}. In task-oriented object detection, the input is typically expressed in terms of ``\textit{affordance}'', denoting an object's capability to support an action or a verb phrase. For example, when tasked with the goal of "sitting comfortably," the robot is expected to identify the most suitable instances depicted in the image. Notably, task-oriented detection algorithms face two distinct challenges, setting them apart from traditional object detection methods. The first challenge is that the object detection model needs to match image patches with text descriptions.
%Firstly, traditional object detection methods are not focused on learning a direct mapping between nouns and objects; instead, they aim to establish a mapping between abstract affordances and the visual attributes of objects. 
%Secondly, task-oriented detection grapples with inherent ambiguity.

As illustrated in Fig.~\ref{fig: motivation}(a), consider the task of finding an object suitable for ``sitting comfortably''. In the left panel, a sofa is a preferable choice due to its ergonomic design and armrests, as compared with a bed. 
However, in the right panel, when no sofa is present in the image, the bed becomes the more suitable candidate. 
In essence, objects that afford a particular verb exhibit ambiguity, necessitating the algorithm to model preferences.

Recently, Large Language Models (LLMs) like GPT-3 \cite{brown2020language} and ChatGPT \cite{ouyang2022training} have showcased remarkable abilities in encoding comprehensive world knowledge acquired from extensive textual data. 
One rudimentary approach to adapt task-oriented detection to traditional object detection involves instructing LLMs to provide a list of objects suitable for a given task, expressed as ``Give a list of objects to fulfill the task \underline{\hspace{1cm}}''.
However, we have observed that LLMs tend to return only a limited set of frequently encountered and similar object categories.
Consequently, this approach may overlook less common yet potentially relevant objects that could complete the task, leading to a decline in performance, particularly in challenging scenarios. 
Moreover, the resulting list only contains the name of the objects, and retains the aforementioned ambiguity, resulting in suboptimal choices in certain situations.

\begin{figure}[!t]%
\centering
\includegraphics[width=1\columnwidth]{figures/motivation.pdf}
\caption{(a) Task-oriented object detection example. (b). Large Vision-Language model example. (3) The most challenging part of task-oriented object detection.} \label{fig: motivation}
\end{figure}

Given the limitations highlighted above, our pursuit of solutions takes cues from the problem-solving capabilities of humans. 
When humans tackle tasks, they follow a multi-step process. 
Initially, they identify all potential instances relevant to the task and proceed to extract their visual attributes. 
Simultaneously, humans parse the task, discerning the required attributes essential for task completion. 
Subsequently, they evaluate instances against these task-relevant attributes, selecting those instances that align most closely with the task's requirements. 
Crucially, humans do not merely seek instances directly matching the task; instead, they engage in a reasoning process that considers both instances and the task's attribute prerequisites.

Inspired by this human problem-solving approach, we introduce a neuro-symbolic framework aimed at emulating human-style task-solving. 
Our model begins by localizing all potential instances within the given context and generating embeddings for each instance. 
Additionally, the model parses the task, generating embeddings for the attributes essential for task fulfillment. 
With these instance and task attribute embeddings in hand, the model computes an affinity matrix and utilizes it to predict the optimal selections. 
Benefiting from the advancements in text-image multimodal models, the embedding spaces for text and visuals have already been harmonized. 
An example of such a model is illustrated in Fig.~\ref{fig: motivation}(b). 
Given input images, the model calculates an affinity matrix between the images and the textual descriptions, aiming to maximize the similarity between the embeddings of real image-text pairs while minimizing the similarity of incorrect pairings.
However, a standard text-image multimodal model, while proficient in alignment, falls short of the reasoning capabilities required for selecting the most suitable objects. 
Moreover, these models primarily focus on aligning nouns with objects, often overlooking the mapping from abstract concepts, such as adjectives, to objects. 
In response, we introduce an additional transformer component following the multimodal model, enhancing its performance in handling adjective embeddings.
The proposed neuro-symbolic framework aims to bridge this gap and replicate human-style reasoning for more effective task-oriented object detection.

In particular, this work makes the following contributions:
\begin{itemize}
    \item 1
    \item 2
    \item 3
\end{itemize}
